Do Offline Metrics Predict Online Performance in Recommender Systems?

Recommender systems operate in an inherently dynamical setting. Past recommendations influence future behavior, including which data points are observed and how user preferences change. However, experimenting in production systems with real user dynamics is often infeasible, and existing simulation-based approaches have limited scale. As a result, many state-of-the-art algorithms are designed to solve supervised learning problems, and progress is judged only by offline metrics. In this work we investigate the extent to which offline metrics predict online performance by evaluating eleven recommenders across six controlled simulated environments. We observe that offline metrics are correlated with online performance over a range of environments. However, improvements in offline metrics lead to diminishing returns in online performance. Furthermore, we observe that the ranking of recommenders varies depending on the amount of initial offline data available. We study the impact of adding exploration strategies, and observe that their effectiveness, when compared to greedy recommendation, is highly dependent on the recommendation algorithm. We provide the environments and recommenders described in this paper as Reclab: an extensible ready-to-use simulation framework at https://github.com/berkeley-reclab/RecLab.

==> metrics.tex <==
\section{Evaluation Procedure} 
Given an environment and a recommender we perform the following steps:
\subsection{Offline tuning}
We sample uniformly a set $\Omega_0$ of initial observed user-item pairs. We tune the hyperparameters of the recommender algorithms to minimize a metric (typically RMSE) on $\Omega_0$. In our experiments $n_{users} = 1000$, $n_{items} = 1700$ and $|\Omega_0|=100000$, which is less than 6\% of the full rating matrix. We choose these settings since they are comparable in size with the popular MovieLense 100K benchmark dataset.
\subsection{Online updates}
A online trial consists of $T$ timesteps. At time $t$, the environment samples uniformly a set of online users. Denote by $\Omega_t$ the set of historical user-item ratings up to time $t$. Using the hyperparameters tuned on the offline snapshot we perform full retraining of the recommendation algorithm on the set $\Omega_t$. Subsequently the online users receive recommendations according to the re-trained recommender and reveal noisy versions of the ground truth ratings. Let $\hat r_t(u,i)$ be the predicted rating associated to user $u$ and item $i$, and $r_t(u,i)$ be the observed ratings.  In static environments $\mathbb{E}r_t(u, i) = r(u, i) \forall t$, whereas in dynamic environment user preferences change in response to previous recommendations. Denote by $\Gamma_t$ be the set of new user-item ratings obtained trough this interaction. Throughout a trial the set of observed ratings is increasing as follows: $\Omega_{t+1} = \Omega_t \cup \Gamma_t$.

\subsection{ Evaluation Metrics}

Online performance of algorithms is evaluated in two settings: \emph{observed} and \emph{population}. As the name suggests, the observed performance refers to metrics computed on the observed user-item pairs. Running experiments in a simulation environment grants us access to ground truth ratings for unobserved items thus by population evaluation we refer to metrics computed on the full rating data. The metrics we consider are:
\begin{itemize}
    \item \textit{RMSE}: The root mean squared error at time $t$ with respect to an index set $\Omega$ is defined as:
\begin{equation*}
    RMSE_t(\Omega) = \sqrt{\frac{1}{|\Omega|}\sum_{(u, i) \in \Omega} (r_t(u,i) - \hat r_t(u,i))^2}
\end{equation*}
RMSE is the most common metric for training and  evaluating prediction based recommenders.

\item \textit{Mean Rating}:
The mean underlying rating at time $t$ with respect to an index set $\Omega$ is computed as:
\begin{equation*}
    MR_t(\Omega) = \sqrt{\frac{1}{|\Omega|}\sum_{(u, i) \in \Omega} (r_t(u,i))}
\end{equation*}
An increase to the Mean Rating statistic on the observed ratings $\Gamma_t$ indicates that the recommender is learning to select highly rated items. A decreasing Mean Rating could either indicate that performance is deteriorating or that the environment is running out of highly rated items. To exclude the former we limit the number of iterations in a trial such that there always remain items that would be rated highly by each user.

\item \textit{nDCG@k}:
Normalized Discounted Cumulative Gain (nDCG) is a measure of ranking quality.  Discounted Cumulative Gain adds up the true ratings up to position $k$ with a  logarithmic penalty proportional to the position of the item relative to predicted ratings. Assuming that $\hat\pi(i)$ is the order of items according to predicted ratings ($\hat\pi(i) = i'$ means that the item $i'$ is ranked in position $i$). Similarly $\pi(i)$ is the ordering of items according to true ratings. DCG  and Idealized DCG can the computed as:
\begin{equation*}
    DCG@k(\Omega) = \sum_{u\in \Omega} \sum_{i=1}^k \frac{r_t(u,\hat\pi(i))}{\log_2(i+1)} \qquad \qquad IDCG@k(\Omega) = \sum_{u\in \Omega} \sum_{i=1}^k \frac{r_t(u,\pi(i))}{\log_2(i+1)}
\end{equation*}
Then nDCG is the ratio of the two: $nDCG@k(\Omega) = \frac{DCG@k(\Omega)}{IDCG@k(\Omega)}$




\item \textit{Other metrics} 

Beyond accuracy, the main metrics in recommender systems research fall into four main categories: novelty, diversity, serendipity, and coverage \cite{herlocker, kaminskaseval}. Diversity generally refers to intra-list heterogeneity of recommended items. Diversity is not well-suited for our setting, since we focus on top-1 recommendation.

Novelty and serendipity are closely related concepts. Novelty is the difference of recommendations at a timestep when compared to previously seen recommendations. Serendipity is the combination of novelty with relevance to the user. Adapting our metric from Kaminskas and Bridge \cite{kaminskaseval}, the novelty of a recommender at timestep $t$ is:

\begin{equation}
    Novelty_t = \frac{-\sum_{i \in \Gamma_t} log_2(p_i)}{\vert \Gamma_t \vert}
\end{equation}

Where $p_i$ is $\frac{\{\vert u \in U, r_{ui} \neq \emptyset \}}{\vert U \vert}$ and U refers to the set of all users in the environment. This represents the running popularity of an item. $\Gamma_t$ represents the set of recommendations at timestep $t$.

Lastly, coverage refers to the percentage of all items that the model recommends to online users. A simple definition is coverage is the number of unique recommended items at each timestep.

TODO: Analyze the correlation between novelty, coverage, and accuracy based on experiments in our environments. Suggest future directions for ways to measure serendipity. Diversity is beyond the scope of this work. 
\end{itemize}


\begin{comment}
\subsection{Regret}
Regret measures the sum of cumulative differences in performance between a model and the best action in hindsight. We compute regret with respect to the oracle model as follows: 
\begin{equation*}
    Regret_t(\Gamma_t) =\sum_{(i,j)\in \Gamma_t}(r^*_t(u,i) - r_t(u,i))
\end{equation*}
Where $r^*$ are the ratings corresponding to the Oracle Model. \mc{$r^*$ is kinda like $r$, except for additive noise, I need to make this distinction more clear}. The cumulative regret is the sum of regret terms up to time $t$:
\begin{equation}
    CummulativeRegret_T = \sum_{t=1}^T Regret_t(\Gamma_t)
\end{equation}
\end{comment}
